Social distancing in networks: A web-based interactive experiment

Governments have used social distancing to stem the spread of COVID-19, but lack evidence on the most effective policy to ensure compliance. We examine the effectiveness of fines and informational messages (nudges) in promoting social distancing in a web-based interactive experiment conducted during the first wave of the pandemic on a near-representative sample of the US population. Fines promote distancing, but nudges only have a marginal impact. Individuals do more social distancing when they are aware they are a superspreader. Using an instrumental variable approach, we argue progressives are more likely to practice distancing, and they are marginally more responsive to fines.

==> chapters/instructions.tex <==
Section \ref{sec:instructions_main_experiment} presents instructions and the interface for the experiment. Analogously, Sections \ref{sec:instructions_svo} and \ref{sec:instructions_bret} present instructions and the interface for the social preferences (SVO) and risk preferences (BRET) elicitation tasks respectively.

\subsection{Main Experiment}
\label{sec:instructions_main_experiment}

This section contains instructions for the Baseline and Intervention parts of the experiment. For the Baseline (Part 1), the rate of contagion is set at 65\%. Note that the type of network and intervention do not feature in this part of instructions. For the Intervention (Part 2), we show instructions for the fine. Instructions for the nudge are similar, except that instead of explaining how the fine is implemented, participants are asked to watch a 3-minute video. The video can be accessed online at \url{https://youtu.be/tyf6EpSMeGs}. The section concludes with \Cref{fig:experiment_interface}, which shows the decision and results interfaces from the main experiment. 

\textbf{Part 1: Instructions (page 1/6)}

Welcome to this interactive experiment!

This experiment consists of two parts. You will be paid a \textbf{fixed reward of \$1} for completing all parts of the experiment. Additionally, you can earn points for your choices in Parts 1 and 2, which will be converted into \$ at the end of this experiment. There may also be a Bonus Task at the end of the experiment.

In Parts 1 and 2 of the experiment, you will \textbf{interact with a group of other real people recruited through MTurk}. Recall that you will never learn the identities of other people and no one will learn about your identity.

The expected duration of the experiment is \textbf{30-40 minutes} and your average expected total earnings will be \textbf{\$3-6 excluding the Bonus Task}. Note that you can earn less or more than this amount depending on your choices and the choices of others in your group.

At the beginning of Part 1 of the experiment, you will be randomly allocated to a \textbf{group of 5} and you will \textbf{remain in this group} for the duration of Parts 1 and 2 of the experiment. Note that you might have to wait while we are matching you with 4 other people, but we will compensate you for the time you wait.

Since this experiment is interactive, it is important that you \textbf{remain continuously attentive}, otherwise you may slow down others and may even be disqualified from the experiment.

In Part 1 of the experiment, you will be asked to play a game with the other members of your group. The instructions on the next 5 pages explain the rules of the game. You will receive more information about Part 2 after you complete Part 1.

All participants are given the \textbf{same} instructions. It is important that you read these instructions carefully. Note that there is no deception in this experiment.

Once you read the instructions, you will be required to pass a short understanding Quiz. \textbf{If you fail the Quiz, you will not be allowed to take part in the experiment and will not receive the fixed reward.}

To continue to the instructions, press the Next button below.

\textbf{Part 1: Instructions (page 2/6)}

In Part 1 of the experiment you are asked to play a game with the other members of your group. In what follows, you and the other members of your group are referred to as participants.

At the start of the game, you are presented with a diagram with 5 circles labeled by capital letters (P, E, C, M, Q) and lines between them.

Each circle represents a \textbf{position} -- one for each participant. At the start of the game, each participant is \textbf{randomly allocated} to one of these positions in the diagram. Your position is the one colored in blue.

The lines between positions indicate the structure of interactions between participants in these positions. These lines \textbf{indicate which participants interact} with one another in the game.

An example is the diagram below. Here, you are in position M and directly interact with participants in positions P and E, but you do not interact directly with C and Q.

\vspace{0.3cm}
\centerline{\includegraphics[scale=.5]{example_network.png}}

The next page of the instructions explains the choice you need to make in the game.

To continue to the next page, press the Next button below. To go to the previous page, press the Back button.

\textbf{Part 1: Instructions (page 3/6)}

In the game, you and the other participants face a \textbf{risk of getting infected with COVID-19} (commonly known as coronavirus).

The main symptoms of COVID-19 are shortness of breath, a high fever and a new, continuous cough. Most patients experience mild symptoms and recover in 1-2 weeks, but cases can progress to pneumonia and organ failure in the most vulnerable individuals.

After you learn your position in the diagram, your need to \textbf{choose whether to practice social distancing}. Below you can see what the buttons to make your choice look like.

\vspace{0.3cm}
\centerline{\includegraphics[scale=.75]{images/interface_buttons.png}}

You have \textbf{20 seconds} to make your choice and the timer is displayed at the top of the interface throughout the experiment. If you do not make a choice within the allowed time, your choice is automatically recorded as a ‘No’.

After everyone in your group has made their social distancing choice, the computer randomly chooses \textbf{one and only one participant to contract COVID-19 directly}. If a participant does not practice social distancing and is randomly picked by the computer then s/he gets infected for sure. In other words, \textbf{if you do not practice social distancing there is a 20\% chance you get infected with COVID-19 directly}.

Social distancing gives you some level of protection against COVID-19. If you practice social distancing and you are the participant randomly chosen by the computer to be infected then the computer flips a fair coin. If the coin flip is Head you are infected with COVID-19. If the coin flip is Tail then you are not infected with COVID-19. In other words, \textbf{if you practice social distancing there is a 10\% chance you get infected with COVID-19 directly}.

A participant who practices social distancing cannot pass COVID-19 to other participants and cannot be infected with COVID-19 by another participant.

On the other hand, an infected participant who does not practice social distancing may infect other participants through contagion. In particular, other participants who do not practice social distancing face a risk of getting infected because COVID-19 may spread through \textbf{interactions} between the participants.

The next page of the instructions explains how COVID-19 spreads through interactions between participants.

To continue to the next page, press the Next button below. To go to the previous page, press the Back button.

\textbf{Part 1: Instructions (page 4/6)}

A healthy participant who does not practice social distancing may get infected with COVID-19 through \textbf{contagion} by interacting with infected participants who do not practice social distancing. The probability a participant contracts COVID-19 through interaction with another participant is referred to as the \textbf{rate of contagiousness} of COVID-19.

\textbf{Throughout Part 1 of the experiment the rate of contagiousness of COVID-19 is fixed at 65\%.}

Consider again the example diagram of interactions and, as an example, suppose that:

\vspace{0.3cm}
\centerline{\includegraphics[scale=.5]{example_network.png}}

\begin{itemize}
    \item You (participant M) do not practice social distancing.
    \item Participants in position E and Q practice social distancing, while participants in positions P and C do not.
\end{itemize}

In this example, suppose C is randomly picked by the computer to contract COVID-19 directly.

First, C has chosen not to practice social distancing so s/he gets infected for sure. Moreover, C can pass COVID-19 to other participants because s/he does not practice social distancing.

Second, E and Q cannot get infected with COVID-19 through contagion because they practice social distancing.

Next, P may get infected through contagion because s/he does not practice social distancing and interacts with C. This can happen with probability 65\% -- the rate of contagiousness.

Finally, you may also become infected by contagion through your interaction with P. Specifically, there is a 65\% probability you might get infected through your interaction with P if s/he becomes infected. However, if P remains healthy you will also remain healthy for the duration of the game.

It follows that in this example if 1) you do not practice social distancing, 2) E and Q practice social distancing whereas P and C do not, and 3) C contracts COVID-19 directly, then you may become infected with probability 42.25\%. The diagram below shows how this percentage is computed.

\vspace{0.3cm}
\centerline{\includegraphics[scale=.75]{images/65_percent.png}}

Note that you will not be informed of the choices of other participants at any point during the experiment.

The next page of the instructions explains how you earn points in Part 1 of the experiment.

To continue to the next page, press the Next button below. To go to the previous page, press the Back button.

\textbf{Part 1: Instructions (page 5/6)}

At the end of the game you earn the following points depending on your social distancing choice and infection status:

\begin{itemize}
    \item \textbf{100 points:} if you did not practice social distancing and did not get infected;
    \item \textbf{65 points:} if you practiced social distancing and did not get infected (100 points for being healthy minus 35 points cost of social distancing);
    \item \textbf{0 points:} if you did not practice social distancing and got infected;
    \item \textbf{-35 points:} if you practiced social distancing and got infected (0 points for being infected minus 35 points cost of social distancing).
\end{itemize}

Note that \textbf{if you fail to submit} your social distancing choice then you will receive a \textbf{penalty of 200 points}.

The information about the points you can earn, the rate of contagiousness of COVID-19, the structure of interactions between participants and your position are always displayed on the screen when you make your social distancing choice.

Below you can see an example of how this part of the interface looks like. The diagram of interactions is on the right, while the textual information on the left reminds you of the rate of contagiousness and the possible outcomes.

\vspace{0.3cm}
\centerline{\includegraphics[scale=.75]{images/interface_decision.png}}

At the end of the game, you are reminded of the structure of interactions between participants, your position within that structure, and your social distancing choice. You are also informed of your infection status and the number of points earned.

Below you can see an example of how this part of the interface looks like.

\vspace{0.3cm}
\centerline{\includegraphics[scale=.75]{images/interface_results.png}}

You have 15 seconds to review this information and the timer is always displayed at the top of the interface.

The next page of the instructions explains how points are converted into your earnings in \$.

To continue to the next page, press the Next button below. To go to the previous page, press the Back button.

\textbf{Part 1: Instructions (page 6/6)}

Part 1 of the experiment has \textbf{20 separate games} as described in these instructions. \textbf{The choice you make in one game has no effect on other games.}

The only variation between games is the random reassignment of the positions of all the participants (including you) in the diagram of interactions. The participants assigned to your group, the structure of interactions between positions, the probability of contracting COVID-19 directly, the rate of contagiousness of COVID-19 and the number of points earned depending on social distancing choice and infection status remain unchanged.

At the end of each game, you can review the history of your choices and outcomes for the last 5 games. The table below shows an example of how your history after 9 games might look like.

\vspace{0.3cm}
\centerline{\includegraphics[scale=.75]{images/interface_history.png}}

It is important that you make a choice in every game. If you fail to make a choice for \textbf{3 consecutive games}, you will be \textbf{disqualified from the experiment}. In this case, you will not receive any payment for this experiment.

At the end of this experiment, the computer randomly picks \textbf{4 out of 20 games} to determine your earnings for Part 1 of the experiment.

\textbf{The points are converted to \$ at a rate of 115 points per \$1.}

Suppose that you earn 260 points in the 4 randomly drawn games. Then, your total earnings for Part 1 are \$2.26.

To continue to the short Quiz, press the Next button below. To go to the previous page of the instructions, press the Back button.

\textbf{Part 2: Instructions}

You have completed Part 1 of the experiment and will now proceed to Part 2.

Below are the instructions for Part 2 of the experiment. It is important that you read these instructions carefully.

This part of the experiment also has 20 games, and you are assigned to the same group of 5 people as in Part 1. The structure of interactions between participants, the probability of contracting COVID-19 directly and the rate of contagiousness of COVID-19 are the same as in Part 1.

\textbf{The single difference from Part 1 is that in Part 2 of the experiment you will receive a fine of 15 points in any game in which you do not practice social distancing.}

Hence, in Part 2 of the experiment the points you earn at the end of the game are:

\begin{itemize}
    \item \textbf{85 points:} if you did not practice social distancing and did not get infected (100 points for being healthy minus 15 points fine);
    \item \textbf{65 points:} if you practiced social distancing and did not get infected (100 points for being healthy minus 35 points cost of social distancing);
    \item \textbf{-15 points:} if you did not practice social distancing and got infected (0 points for being infected minus 15 points fine);
    \item \textbf{-35 points:} if you practiced social distancing and got infected (0 points for being infected minus 35 points cost of social distancing).
\end{itemize}

Note that if you fail to submit your social distancing choice then you will receive a penalty of 200 points.

Your earnings for Part 2 are computed in the same way as in Part 1. At the end of this experiment, the computer randomly picks 4 out of 20 games to determine your earnings for Part 2 of the experiment.

As in Part 1, the points are converted to \$ at a rate of \textbf{115 points per \$1.}

Suppose that you earn 300 points in the 4 randomly drawn games. Then, your total earnings for Part 2 are \$2.61.

Before you can start Part 2 of the experiment, you must answer a \textbf{Quiz question on the instructions above}. If you fail to answer the question correctly, you will not be able to continue to Part 2 of the experiment.

To continue to the short Quiz, press the Next button below.

\textbf{The experiment: Interface}

\Cref{fig:experiment_interface} shows the decision and results interface from the main experiment. We focus on game 5 of the Intervention part of the experiment, where the rate of contagion is set at 65\%, the network is the star, and fine is the intervention. In this game, our example participant is assigned to position P. She decides to practice social distancing, and does not get infected. 

\begin{figure}[!ht]
\begin{minipage}{\linewidth}
\centering
\subfloat[Decision interface]{\label{fig:decision_interface}
\includegraphics[width=0.95\textwidth]{images/interface_decision_full.png}
}
\end{minipage}
\begin{minipage}{\linewidth}
\centering
\subfloat[Results interface]{\label{fig:results_interface}
\includegraphics[width=0.95\textwidth]{images/interface_results_full.png}
}
\end{minipage}
\caption{Game 5 of the Intervention: interface}
\label{fig:experiment_interface}
\end{figure}

\subsection{Social Value Orientation (SVO) Slider Measure}
\label{sec:instructions_svo}

This section contains instructions from and interface of the Social Value Orientation (SVO) task which participants complete as part of the recruitment survey. 

\textbf{SVO: Instructions}

You have answered the qualifying questions correctly and are now in the Bonus Task.

In this Bonus Task you will be making a series of decisions about allocating money between you and another anonymous Turker (hereafter, Other). All of your decisions will be completely confidential.

There is a total of 6 decisions to make which are independent of each other. For each decision, you are asked to pick the distribution of money between yourself and Other that you prefer, all values are stated in cents. After you have made your decision, select the resulting distribution of money by clicking on the button below your choice. As you will see, your choices will influence both the amount of money you receive as well as the amount of money the Other receives.

There are no right or wrong answers, this is all about personal preferences.

Every time 50 Turkers complete the task, we will randomly pick two of them and pay them for the Bonus Task as follows. We will pick one of the 6 decisions, and randomly implement the decision of one of the two chosen Turkers.

For example, suppose we randomly chose Turkers X and Y out of those 50 Turkers, and that we further randomly chose to implement decision 3 of Turker Y. Suppose that in decision 3 Turker Y allocated 150 cents to themselves, and 140 cents to Other. Therefore, Turkers X and Y will be paid 140 and 150 cents respectively.

\textbf{SVO: Interface}

\Cref{fig:svo_interface} presents part of the interface of the SVO task. We focus on one of the six decisions. In this example, a participant decided to allocate 288 cents to self and 188 cents to other.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.9\textwidth]{images/svo_choice.png}
    \caption{Social Value Orientation (SVO) Slider Measure: Decision interface}
    \label{fig:svo_interface}
\end{figure}

\subsection{Bomb Risk Elicitation Task (BRET)}
\label{sec:instructions_bret}

This section contains instructions from and interface of the Bomb Risk Elicitation Task (BRET) which participants complete after the main experiment.

\textbf{BRET: Instructions}

Thank you very much for taking part in the experiment!

You are now in the Bonus Task in which you have an opportunity to earn an extra payment.

On the next page, you will see 100 boxes. As soon as you start the task by pressing the \textbf{`Start'} button, one box is collected per second starting from the top left corner. Once collected, the box is marked by a tick symbol.

\textbf{For each box collected, you earn 2 cents.}

One of the 100 boxes contains a \textbf{bomb} that destroys all of your earnings. \textbf{You do not know where the bomb is located.} You only know that the bomb can be in any box with equal probability.

Your task is to choose when to stop collecting the boxes and open those you have collected. You stop collecting boxes by pressing \textbf{`Stop'} at any time. After that you open the boxes you have collected by pressing the \textbf{`Open'} button. Note that once you press `Stop' you cannot restart collecting boxes.

A dollar or a bomb symbol will be shown on each of the boxes you have collected.

If the bomb symbol does not appear, that means that you have \textbf{not collected the box with the bomb}. In this case, you \textbf{earn the amount accumulated by the boxes you have collected}.

If the bomb symbol appears, that means that you \textbf{have collected the box with the bomb}. In this case, you \textbf{earn zero} for the Bonus Task.

To proceed to the Bonus Task, press the button below.

\textbf{BRET: Interface}

\Cref{fig:bret_interface} presents the interface of the BRET. \Cref{fig:bret_choice} shows an example of the interface after a participant has stopped collecting boxes. We can see that she opened 56 boxes. \Cref{fig:bret_result} shows the interface after she opened the boxes. We can see that the bomb is among the 56 collected boxes. Consequently, in this example the participant earns zero for the BRET. 

\begin{figure}[ht]
\begin{minipage}{.5\linewidth}
\centering
\subfloat[Decision interface]{\label{fig:bret_choice}
\includegraphics[scale=0.6]{images/bret_choice.png}
}
\end{minipage}
\begin{minipage}{.5\linewidth}
\centering
\subfloat[Results interface]{\label{fig:bret_result}
\includegraphics[scale=0.6]{images/bret_result.png}
}
\end{minipage}
\caption{Bomb Risk Elicitation Task (BRET) interface}
\label{fig:bret_interface}
\end{figure}


==> chapters/robustness.tex <==
This section presents additional statistical analysis. Section \ref{sec:robustness_convergence} presents convergence analysis for Baseline and Intervention. Section \ref{sec:robustness_aggregate} summarizes robustness checks performed at the aggregate (group) level, and Section \ref{sec:robustness_individual} focuses on robustness checks at the individual level.

\subsubsection{Aggregate analysis} 
\label{sec:robustness_aggregate}

We test the robustness of findings in Section \ref{sec:analysis_aggregate} in two ways: (1) using data from all 20 rounds of both parts of the experiment, and (2) employing parametric rather than non-parametric tests on the data from the last 10 rounds of both parts. \Cref{tab:nonparametric_robustness} summarizes the results of these robustness checks.

In the columns under `Robustness \#1', we present the results of our hypothesis tests when using decision data from all rounds. From the tables, we can see that most of the results from Section \ref{sec:analysis_aggregate} are robust to using data from all 20 rather than the last 10 rounds of both parts of the experiment. Further, recall that we observed previously that the nudge effects appear to be small and sensitive to specification. Part 3 of \Cref{tab:nonparametric_robustness} provides further evidence strengthening this observation -- we see that the effect of the nudge on distancing levels is now insignificant in most of the specifications.

In our second robustness check, we use the standard unpaired t-test (UT) on unmatched samples instead of the MW test, and the paired version of the t-test (PT) on matched samples in place of the WSR test. In the columns under `Robustness \#2' of \Cref{tab:nonparametric_robustness}, we repeat the analysis from Section \ref{sec:analysis_aggregate} using these parametric tests. Comparing the tables, we can see that all significant effects are still present if we use parametric rather than non-parametric tests.

Overall, the findings of this section suggest that the observations made in Section \ref{sec:analysis_aggregate} are robust to changes in the distributional assumptions of the tests, and inclusion of all observations.

\input{tables/nonpar_robustness}

\subsubsection{Individual analysis} \label{sec:robustness_individual}

We now test the robustness of the parametric analysis in Section \ref{sec:analysis_individual}. Model 1 of Table \ref{tab:logit_robustness} restates our preferred specification to aid comparison. Models 2 and 3 vary the type of model: they use a Linear Probability Model (LPM) and a Probit model, respectively. Both include random effects, to allow for individual heterogeneity. Changing the type of model used does not materially affect the results. Note that the coefficients are not directly comparable across Logit, LPM, and Probit. Figure \ref{fig:ape_robust} shows the average partial effects under each type of model -- as we can see, the differences are small. Model 4 shows that our results are not sensitive to excluding the period before subjects converge -- they are little affected by including all rounds. 

The results could also be driven by subjects who either might not be paying attention or who might have a poor understanding of the game. To test for this, we exclude any subjects who chose to practice social distancing in all 40 rounds (there are 122 subjects who do this) in model 5. Then in model 6, we exclude subjects failing the quiz between the two parts of the experiment more than once, or who failed the post-experiment attention check.\footnote{A question in the post-experiment survey asked subjects to select a particular option to demonstrate that they were paying attention.} 

Finally, Model 7 tests an alternative specification of the instrument -- only using subjects' responses to the question of whether global warming is caused by humans.\footnote{Using the final question on its own also gives similar results in terms of magnitude and statistical significance. The question regarding whether global warming is happening gives non-significant estimates -- likely driven by the fact that there is very little variation in the responses to this question. 353 (out of 394) subjects respond that global warming is happening.}

While clearly not definitive, these suggest that our findings are robust, and in particular are not driven by the choices we made on the econometric model and which, if any, observations to exclude.

In our main analysis, we used an ideology index, constructed from subjects' responses to questions immediately asked after the experiment. \Cref{tab:political_party_robustness} shows that these results hold even if we use political party affiliation -- a much coarser, but much more widely available, measure of ideology. Apart from the ideology control, all variables are the same as in the main model, so we suppress them in the table for convenience. Model 1 shows the main Random Effects Logit model for reference. Model 2 uses dummies for self-identified Republicans, and `Other' (leaving self-identified Democrats as the base category). Model 3 omits the `Other' category -- leaving a direct comparison of Republicans and Democrats. Model 4 uses the instrumental variables method. Note that we only have one instrument, so it is not possible to instrument for both Republicans and Independents in the same regression. 

Our preferred specification only contains a single type of heterogeneous treatment effect -- the effect of the fine varies with subjects' ideology. There also appear to be some other interaction effects present. \Cref{tab:logit_heterogenous} summarizes heterogeneous treatment effects. Older subjects are \emph{relatively less} responsive to the fine (REL, $p<0.0001$); although the fine does still increase their probability of social distancing (REL, $p<0.0001$). Prosocial subjects are also marginally less responsive to the fine (REL, $p=0.07$). Subjects in a high contagion setting, and older subjects are \emph{relatively more} responsive to the nudge (REL, $p=0.006$ and $p=0.02$ respectively). This suggests that the impact of policy interventions may vary across groups, and perhaps more importantly may vary with how contagious the disease is.
\clearpage

\input{tables/robustness_checks_1.tex}
\clearpage

\input{tables/political_party_logit.tex}
\clearpage

\input{tables/heterogeneous_regs}

==> tables/convergence.tex <==
\begin{table}[ht]
\centering
\begin{threeparttable}
\caption{Individual convergence analysis.}
\label{tab:convergence}
% \begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{ccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{2cm}{Network}} & \multicolumn{1}{c}{\multirow{2}{2.5cm}{\begin{tabular}[c]{@{}c@{}}Type of \\ intervention\end{tabular}}} & \multicolumn{1}{c}{\multirow{2}{1cm}{n}} & \multicolumn{1}{c}{\multirow{2}{3cm}{\begin{tabular}[c]{@{}c@{}}$>$80\% converged\\ by round ...\end{tabular}}} & \multicolumn{1}{c}{\multirow{2}{3cm}{\begin{tabular}[c]{@{}c@{}}...\% converged \\ by round 11\end{tabular}}} \\
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \\
\midrule
% Part 1
\multicolumn{5}{l}{\textbf{Baseline}} \\ \hline
all & all & 400 & 9 & 84.25 \\ \hline
complete & all & 200 & 8 & 86 \\ 
star & all & 200 & 11 & 82.5 \\ \hline
% Part 2
\multicolumn{5}{l}{\textbf{Intervention}} \\ \hline
all & all & 400 & 7 & 87.5 \\ \hline
complete & all & 200 & 6 & 89.5 \\ 
star & all & 200 & 9 & 85.5 \\ \hline
all & fine & 200 & 7 & 90 \\ 
all & nudge & 200 & 8 & 85 \\ \hline
\multirow{2}{*}{complete} & fine & 100 & 6 & 92  \\ & nudge & 100 & 6 & 87 \\
\multirow{2}{*}{star} &  fine & 100 & 7 & 88 \\ & nudge & 100 & 9 & 83 \\ 
\bottomrule
\end{tabular}
% \begin{tablenotes}
%     %   \small
%       \item 
% \end{tablenotes}
\end{threeparttable}
\end{table}

==> tables/heterogeneous_regs.tex <==

\setlength\LTleft{-10mm}
\begin{ThreePartTable}
% \renewcommand\TPTminimum{\textwidth}
%% Arrange for "longtable" to take up full width of text block
% \setlength\LTleft{0pt}
% \setlength\LTright{0pt}
% \setlength\tabcolsep{0pt}
\begin{TableNotes}
  \item [a] -- all other controls from the main model.
  \item Significance levels: * -- 10\%, ** -- 5\%, *** -- 1\%.
  \item Specification is same as main model except for the interaction term. Instead of interacting policy interventions with ideology, they are interacted with the variable in the column heading.
\end{TableNotes}
\begin{longtable}{ladadad}
\caption{Checks for heterogeneous treatment effect.}
\label{tab:logit_heterogenous} \\
\toprule
&  \multicolumn{6}{c}{Decision to practice distancing (binary)} \\ \cline{2-7} 
\multicolumn{1}{c}{Variables} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}High\\Contagion \end{tabular}} & \multicolumn{1}{c}{Peripheral} & \multicolumn{1}{c}{Superspreader} & \multicolumn{1}{c}{Age} & \multicolumn{1}{c}{Prosocial} & \multicolumn{1}{c}{Risk}\\
\midrule
\endfirsthead
\multicolumn{7}{c}{\textit{Continued from previous page}} \\
\toprule
&  \multicolumn{6}{c}{Decision to practice distancing (binary)} \\ \cline{2-7} 
\multicolumn{1}{c}{Variables} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}High\\Contagion \end{tabular}} & \multicolumn{1}{c}{Peripheral} & \multicolumn{1}{c}{Superspreader} & \multicolumn{1}{c}{Age} & \multicolumn{1}{c}{Prosocial} & \multicolumn{1}{c}{Risk}\\
\midrule
\endhead
\multicolumn{7}{r}{\textit{Continued on next page}} \\
\endfoot
\hline
\insertTableNotes 
\endlastfoot
Fine & 0.475 & 0.814*** & 0.754*** & 3.023*** & 1.201*** & 1.458** \\
 & (0.336) & (0.273) & (0.252) & (0.515) & (0.333) & (0.590) \\
Nudge & -0.0445 & 0.305 & 0.389** & -0.928 & 0.409** & 0.468 \\
 & (0.225) & (0.206) & (0.159) & (0.582) & (0.208) & (0.405) \\
High contagion & 1.216*** & 1.535*** & 1.538*** & 1.561*** & 1.558*** & 1.538*** \\
 & (0.339) & (0.324) & (0.323) & (0.326) & (0.327) & (0.323) \\
Superspeader & 0.837** & 0.835** & 0.942** & 0.845** & 0.815* & 0.827** \\
 & (0.424) & (0.418) & (0.436) & (0.425) & (0.423) & (0.422) \\
Peripheral & -1.787*** & -1.776*** & -1.785*** & -1.819*** & -1.796*** & -1.789*** \\
 & (0.334) & (0.354) & (0.334) & (0.338) & (0.335) & (0.333) \\
Age (years) & 0.0796*** & 0.0793*** & 0.0793*** & 0.0867*** & 0.0793*** & 0.0794*** \\
 & (0.0138) & (0.0137) & (0.0137) & (0.0142) & (0.0138) & (0.0138) \\
Bomb risk score & -0.0298*** & -0.0297*** & -0.0297*** & -0.0297*** & -0.0301*** & -0.0247*** \\
 & (0.00893) & (0.00891) & (0.00889) & (0.00894) & (0.00890) & (0.00853) \\
Prosocial values & 1.493*** & 1.482*** & 1.488*** & 1.478*** & 1.685*** & 1.483*** \\
 & (0.337) & (0.336) & (0.333) & (0.337) & (0.366) & (0.334) \\
Conservative ideology & -0.283*** & -0.282*** & -0.281*** & -0.278*** & -0.282*** & -0.282*** \\
 & (0.0568) & (0.0565) & (0.0566) & (0.0567) & (0.0565) & (0.0563) \\
Controls$^{\text{a}}$ & Yes & Yes & Yes & Yes & Yes & Yes \\
 &  &  &  &  &  &  \\
\begin{tabular}[c]{@{}l@{}}Interaction with \\ fine treatment \end{tabular} & 0.611 & -0.115 & 0.177 & -0.0505*** & -0.722* & -0.0181 \\
 & (0.482) & (0.458) & (0.595) & (0.0112) & (0.403) & (0.0115) \\
\begin{tabular}[c]{@{}l@{}}Interaction with \\ nudge treatment \end{tabular} & 0.788*** & 0.0870 & -0.496 & 0.0309** & -0.148 & -0.00374 \\
 & (0.288) & (0.292) & (0.381) & (0.0130) & (0.313) & (0.0112) \\
 &  &  &  &  &  & \\
Constant & -1.877 & -2.054 & -2.069 & -2.537 & -2.152 & -2.172 \\
 & (1.665) & (1.665) & (1.670) & (1.722) & (1.673) & (1.685) \\
 &  &  &  &  &  &  \\
Observations & 7,880 & 7,880 & 7,880 & 7,880 & 7,880 & 7,880 \\
No of subjects & 394 & 394 & 394 & 394 & 394 & 394 \\
\bottomrule
\end{longtable}
\end{ThreePartTable}



==> tables/nonpar_robustness.tex <==
% \begin{sidewaystable}[!t]
% \begin{threeparttable}
% \begin{adjustbox}{width=\textwidth,center}
\setlength\LTleft{-10mm}
\begin{ThreePartTable}
% \renewcommand\TPTminimum{\textwidth}
%% Arrange for "longtable" to take up full width of text block
% \setlength\LTleft{0pt}
% \setlength\LTright{0pt}
% \setlength\tabcolsep{0pt}
\begin{TableNotes}
  \item Null Hypothesis: for each hypothesis, sample \#1 and sample \#2 appear consecutively \textit{in italics}; Alt: either 2-sided or 1-sided alternative, a 1-sided alternative is always s.t. median(sample \#1) $>$ median(sample \#2) or mean(sample \#1) $>$ mean(sample \#2) as appropriate; Test: non-parametric: Mann-Whitney U-test (MW) for unmatched samples and Wilcoxon Signed-Rank test (WSR) for matched samples; analogously for parametric: unpaired t-test (UT) and paired t-test (PT); p-val: p-value for the test of the Null Hypothesis against the Alternative; Sig: significance of the test where * -- 10\%, ** -- 5\%, *** -- 1\%.
\end{TableNotes}
\begin{longtable}{lcccaaaddd}
\caption{Robustness checks at the aggregate level, all 20 rounds (Robustness \#1) or last 10 rounds (Robustness \#2) used.}
\label{tab:nonparametric_robustness}\\
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Null Hypothesis}} & \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Rate of \\ contagion\end{tabular}}} & \multicolumn{1}{c}{\multirow{2}{*}{Position}} & \multicolumn{1}{c}{\multirow{2}{*}{Alt}} & \multicolumn{3}{c}{Robustness \#1} & \multicolumn{3}{c}{Robustness \#2} \\
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{Test} & \multicolumn{1}{c}{p-val} & \multicolumn{1}{c}{Sig} & \multicolumn{1}{c}{Test} & \multicolumn{1}{c}{p-val} & \multicolumn{1}{c}{Sig} \\ \midrule
\endfirsthead
\multicolumn{10}{c}{\textit{Continued from previous page}} \\
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Null Hypothesis}} & \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Rate of \\ contagion\end{tabular}}} & \multicolumn{1}{c}{\multirow{2}{*}{Position}} & \multicolumn{1}{c}{\multirow{2}{*}{Alt}} & \multicolumn{3}{c}{Robustness \#1} & \multicolumn{3}{c}{Robustness \#2} \\
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{Test} & \multicolumn{1}{c}{p-val} & \multicolumn{1}{c}{Sig} & \multicolumn{1}{c}{Test} & \multicolumn{1}{c}{p-val} & \multicolumn{1}{c}{Sig} \\ \midrule
\endhead
\multicolumn{10}{r}{\textit{Continued on next page}} \\
\endfoot
\hline
\insertTableNotes 
\endlastfoot
\multicolumn{10}{l}{Part 1. Baseline} \\
\hline
\multirow{6}{3.5cm}{\textit{Fine} vs \textit{nudge}} & all & all & \multirow{6}{*}{2-sided} & MW & .73 &  & UT &  .38 &  \\
 & all & close-knit & & MW & .82 &  & UT & .85 & \\
 & all & superspreader & & MW & .90 &  & UT & .78 &  \\
 & all & peripheral & & MW & .21 &  & UT & .22 &  \\
 & 15\% & all & & MW & .98 &  & UT & .79 &  \\
 & 65\% & all & & MW & .62 &  & UT & .27 &  \\
 \pagebreak
\multicolumn{10}{l}{Part 2. Intervention vs Baseline. \Cref{theor:fine_intervention} (fine has an effect)} \\ \hline
\multirow{6}{3.5cm}{Fine: \textit{Intervention} vs \textit{Baseline}} & all & all & \multirow{6}{*}{1-sided} & WSR & .003 & *** & PT & .001 & *** \\
 & all & close-knit & & WSR & .04 & ** & PT & .01 & ** \\
 & all & superspreader & & WSR & .08 & * & PT & .05 & * \\
 & all & peripheral & & WSR & .04 & ** & PT & .06 & *  \\
 & 15\% & all & & WSR & .09 & * & PT & .07 & * \\
 & 65\% & all & & WSR & .005 & *** & PT & .002 & *** \\
 \hline
\multicolumn{10}{l}{Part 3. Intervention vs Baseline. \Cref{theor:nudge_intervention} (nudge has an effect)} \\ \hline
\multirow{6}{3.5cm}{Nudge: \textit{Intervention} vs \textit{Baseline}} & all & all & \multirow{6}{*}{1-sided} & WSR & .40 &  & PT & .01 & **  \\
 & all & close-knit & & WSR & .36 &  & PT & .06 & *  \\
 & all & superspreader & & WSR & .05 & * & PT & .39 &  \\
 & all & peripheral & & WSR & .18 &  & PT & .05 & *  \\
 & 15\% & all & & WSR & .20 &  & PT & .48 &  \\
 & 65\% & all & & WSR & .07 & * & PT & .0002 & ***  \\ 
 \hline
\multicolumn{10}{l}{Part 4. Intervention. \Cref{theor:fine_vs_nudge} (fine is more effective than nudge)} \\ \hline
\multirow{6}{3.5cm}{\textit{Fine} vs \textit{nudge}} & all & all & \multirow{6}{*}{1-sided} & MW & .06 & * & UT &  .05 & * \\
 & all & close-knit & & MW & .17 &  & UT & .20 &  \\
 & all & superspreader & & MW & .06 & * & UT & .05 &  ** \\
 & all & peripheral & & MW & .13 &  & UT & .10 &  \\
 & 15\% & all & & MW & .17 &  & UT & .12 &  \\
 & 65\% & all & & MW & .06 & * & UT & .09 & * \\ 
 \hline
\multicolumn{10}{l}{Part 5. Baseline. \Cref{theor:position_effect} (superspreader $>$ close-knit $>$ peripheral)} \\ \hline
\multirow{3}{3.5cm}{\textit{Superspreader} vs \textit{close-knit}} & all & -- & \multirow{3}{*}{1-sided} & MW & .0009 & *** & UT & .01 & ** \\
 & 15\% & -- & & MW & .03 & ** & UT & .08 & * \\
 & 65\% & -- & & MW & .008 & *** & UT & .03 & ** \\ \hline
\multirow{3}{3.5cm}{\textit{Close-knit} vs \textit{peripheral}} & all & -- & \multirow{3}{*}{1-sided} & MW & $<$.0001 & *** & UT &  $<$.0001 & *** \\
 & 15\% & -- & & MW & .002 & *** & UT & .003  & *** \\
 & 65\% & -- & & MW & .0005 & *** & UT & .001 & *** \\ \hline
\multirow{3}{3.5cm}{\textit{Superspreader} vs \textit{peripheral}} & all & -- & \multirow{3}{*}{1-sided} & WSR & $<$.0001 & *** & PT & $<$.0001 & ***  \\
 & 15\% & -- & & WSR & .0002 & *** & PT & .0002 & *** \\
 & 65\% & -- & & WSR & .0001 & *** & PT & $<$.0001 & *** \\ \hline
\multicolumn{10}{l}{Part 6. Intervention. \Cref{theor:position_effect} (superspreader $>$ close-knit $>$ peripheral)} \\ \hline
\multirow{3}{3.5cm}{\textit{Superspreader} vs \textit{close-knit}} & all & -- & \multirow{3}{*}{1-sided} & MW & .003 & *** & UT & .007 & ***  \\
 & 15\% & -- & & MW & .009 & *** & UT & .02 & ** \\
 & 65\% & -- & & MW & .07 & * & UT & .07 & * \\ 
\multirow{3}{3.5cm}{\textit{Close-knit} vs \textit{peripheral}} & all & -- & \multirow{3}{*}{1-sided} & MW & .0004 & *** & UT & .0002 & *** \\
 & 15\% & -- & & MW & .004 & *** & UT & .0003 & *** \\
 & 65\% & -- & & MW & .01 & ** & UT & .02 & ** \\ \hline
\multirow{3}{3.5cm}{\textit{Superspreader} vs \textit{peripheral}} & all & -- & \multirow{3}{*}{1-sided} & WSR & $<$.0001 & *** & PT & $<$.0001 & *** \\
 & 15\% & -- & & WSR & $<$.0001 & *** & PT & $<$.0001 & ***  \\
 & 65\% & -- & & WSR & .001 & *** & PT & .0003 & *** \\
\multicolumn{10}{l}{Part 7. Baseline. \Cref{theor:contagion_effect} (more distancing in high contagion compared to low contagion)} \\ \hline
\multirow{4}{3.5cm}{\textit{65\%} vs \textit{15\%} rate of contagion} & all & all & \multirow{4}{*}{1-sided} & MW & .015 & ** & UT & .005 &***  \\
 & all & close-knit & & MW & .08 & * & UT & .05 & ** \\
 & all & superspreader & & MW & .18 &  & UT & .10 & * \\
 & all & peripheral & & MW & .04 & ** & UT & .02 & ** \\ \hline
\multicolumn{10}{l}{Part 8. Intervention. \Cref{theor:contagion_effect} (more distancing in high contagion compared to low contagion)} \\ \hline
\multirow{4}{3.5cm}{\textit{65\%} vs \textit{15\%} rate of contagion} & all & all & \multirow{4}{*}{1-sided} & MW & .0005 & *** & UT & $<$.0001 & ***  \\
 & all & close-knit & & MW & .008 & *** & UT & .007 & ***  \\
 & all & superspreader & & MW & .23 &  & UT & .09 & *  \\
 & all & peripheral & & MW & .005 & *** & UT & .0004 & ***  \\ \hline
\multicolumn{10}{l}{Part 9. Baseline. \Cref{theor:complete_network} (actual versus equilibrium/efficient outcomes in complete network)} \\ \hline
\multirow{2}{3.5cm}{\textit{Actual} vs \textit{equilibrium}} & 15\% & all & \multirow{2}{*}{1-sided} & MW & $<$.0001 & *** & UT & $<$.0001 & ***  \\
 & 65\% & all & & MW & $<$.0001 & *** & UT & .002 & *** \\ \hline
\multirow{2}{3.5cm}{\textit{Actual} vs \textit{efficient}} & 15\% & all & \multirow{2}{*}{1-sided} & MW & $<$.0001 & *** & UT & $<$.0001 & *** \\
 & 65\% & all & & MW & .04 & ** & UT & .01 & ** \\ \hline
\multicolumn{10}{l}{Part 10. Baseline. \Cref{theor:star_network} (actual versus equilibrium/efficient outcomes in star network)} \\ \hline
\multirow{4}{3.5cm}{\textit{Actual} vs \textit{equilibrium}} & \multirow{2}{*}{15\%} & superspreader & \multirow{4}{*}{1-sided} & MW & $<$.0001 & *** & UT & $<$.0001 & ***  \\
 &  & peripheral &  & MW & $<$.0001 & *** & UT & $<$.0001 & ***  \\
 & \multirow{2}{*}{65\%} & superspreader &  & MW & $<$.0001 & *** & UT & $<$.0001 & ***  \\
 &  & peripheral &  & MW & $<$.0001 & *** & UT & $<$.0001 & ***  \\ \hline
\multirow{2}{3.5cm}{\textit{Actual} vs \textit{efficient}} & \multirow{2}{*}{15\%} & superspreader & \multirow{2}{*}{1-sided} & MW & $<$.0001 & *** & UT & $<$.0001 & ***  \\
 &  & peripheral &  & MW  & $<$.0001 & *** & UT & $<$.0001 & ***  \\
\bottomrule
\end{longtable}
\end{ThreePartTable}


==> tables/political_party_logit.tex <==
\begin{ThreePartTable}
\begin{TableNotes}
  \item [a] -- all other controls from the main model.
  \item Significance levels: * -- 10\%, ** -- 5\%, *** -- 1\%.
\end{TableNotes}
\begin{longtable}[c]{ladad}
\caption{Robustness tests of main specification.}
\label{tab:political_party_robustness} \\
\toprule
&  \multicolumn{4}{c}{Decision to practice distancing (binary)} \\ \cline{2-5} 
\multicolumn{1}{c}{Variables} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}(1)\\Main\end{tabular}} &  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}(2)\\Political Party \end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}(3)\\Omit Others\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}(4)\\ IV\end{tabular}} \\
\midrule
\endfirsthead
\multicolumn{5}{c}{\textit{Continued from previous page}} \\
\toprule
&  \multicolumn{4}{c}{Decision to practice distancing (binary)} \\ \cline{2-4} 
\multicolumn{1}{c}{Variables} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}(1)\\Main\end{tabular}} &  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}(2)\\Political Party \end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}(3)\\Omit  Others\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}(4)\\ IV\end{tabular}} \\
\midrule
\endhead
\multicolumn{5}{r}{\textit{Continued on next page}} \\
\endfoot
\hline
\insertTableNotes 
\endlastfoot

Ideology             & -0.250*** &          &                 &          \\
                     & (0.0591)  &          &                 &          \\
Independent          &           & -0.859   &                 &          \\
                     &           & (0.613)  &                 &          \\
Republican           &           & -0.936** & -1.601**        & -1.976** \\
                     &           & (0.467)  & (0.684)         & (0.921)  \\
Fine--ideology       & -0.110*   &          &                 &           \\
interaction          & (0.0618)  &          &                 &           \\
Nudge--ideology      & -0.0266   &          &                 &           \\
interaction          & (0.0447)  &          &                 &           \\
Fine--Republican     &           & 0.348    & 0.329           & -0.231   \\
interaction          &           & (0.556)  & (0.554)         & (0.336)  \\
Nudge-Republican     &           & -0.249   & -0.231          & 0.328    \\
interaction          &           & (0.336)  & (0.336)         & (0.555)  \\
Fine--Independent    &           & 0.704    &                 &          \\
interaction          &           & (0.541)  &                 &          \\
Nudge--Independent   &           & -0.0360  &                 &          \\
interaction          &           & (0.368)  &                 &         \\
Controls$^{\text{a}}$ & Yes & Yes & Yes & Yes \\
 &  &  &  &  \\
 Observations & 7,880 & 7,880 & 7,880 & 7,880 \\
No of subjects & 394 & 394 & 394 & 394 \\
\bottomrule
\end{longtable}
\end{ThreePartTable}


==> tables/robustness_checks_1.tex <==
% \afterpage{\clearpage
\setlength\LTleft{-15mm}
\begin{ThreePartTable}
% \renewcommand\TPTminimum{\textwidth}
%% Arrange for "longtable" to take up full width of text block
% \setlength\LTleft{0pt}
% \setlength\LTright{0pt}
% \setlength\tabcolsep{0pt}
\begin{TableNotes}
  \item [a] -- all other controls from the main model.
  \item Significance levels: * -- 10\%, ** -- 5\%, *** -- 1\%.
\end{TableNotes}
\begin{longtable}{ladadada}
\caption{Robustness tests of main specification.}
\label{tab:logit_robustness} \\
\toprule
&  \multicolumn{6}{c}{Decision to practice distancing (binary)} \\ \cline{2-8} 
\multicolumn{1}{c}{Variables} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}(1)\\Main\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}(2)\\LPM\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}(3)\\Probit\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}(4)\\All Rounds\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}(5) Not Always\\ Distancing\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}(6)\\$\leq 1$ Quiz Fails\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}(7)\\IV\end{tabular}} \\
\midrule
\endfirsthead
\multicolumn{8}{c}{\textit{Continued from previous page}} \\
\toprule
&  \multicolumn{6}{c}{Decision to practice distancing (binary)} \\ \cline{2-8} 
\multicolumn{1}{c}{Variables} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}(1)\\Main\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}(2)\\LPM\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}(3)\\Probit\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}(4)\\All Rounds\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}(5) Not Always\\ Distancing\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}(6)\\$\leq 1$ Quiz Fails\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}(7)\\IV\end{tabular}} \\
\midrule
\endhead
\multicolumn{8}{r}{\textit{Continued on next page}} \\
\endfoot
\hline
\insertTableNotes 
\endlastfoot
Fine & 1.146*** & 0.0953*** & 0.640*** & 0.969*** & 1.152*** & 1.341*** & 1.148*** \\
 & (0.352) & (0.0279) & (0.196) & (0.297) & (0.350) & (0.409) & (0.352) \\
Nudge & 0.438* & 0.0358* & 0.226 & 0.0771 & 0.429* & 0.776** & 0.436* \\
 & (0.261) & (0.0204) & (0.142) & (0.215) & (0.256) & (0.320) & (0.261) \\
High contagion & 1.547*** & 0.151*** & 0.855*** & 1.236*** & 1.374*** & 1.718*** & 1.542*** \\
 & (0.323) & (0.0303) & (0.187) & (0.286) & (0.284) & (0.340) & (0.323) \\
Superspeader & 0.833** & 0.0777** & 0.416* & 0.614* & 1.521*** & 0.985** & 0.851** \\
 & (0.424) & (0.0329) & (0.235) & (0.347) & (0.390) & (0.475) & (0.429) \\
Peripheral & -1.785*** & -0.174*** & -0.999*** & -1.619*** & -0.999*** & -1.623*** & -1.767*** \\
 & (0.333) & (0.0328) & (0.190) & (0.296) & (0.314) & (0.367) & (0.338) \\
Controls$^{\text{a}}$ & Yes & Yes & Yes & Yes & Yes & Yes & Yes \\
 &  &  &  &  &  &  & \\
Residuals &  &  &  &  &  &  & -0.0809 \\
 &  &  &  &  &  &  & (0.120) \\
Constant & -2.213 & 0.284* & -1.192 & -1.380 & -3.481** & -3.439* & -2.487 \\
 & (1.666) & (0.151) & (0.960) & (1.483) & (1.370) & (1.880) & (1.722) \\
 &  &  &  &  &  &  & \\
Observations & 7,880 & 7,880 & 7,880 & 15,760 & 5,440 & 6,340 & 7,880 \\
No of subjects & 394 & 394 & 394 & 394 & 272 & 317 & 394 \\
\bottomrule
\end{longtable}

\vspace*{0.3cm}  % set amount of vertical offset

\includegraphics[width=\textwidth]{images/fig4.pdf}
\captionof{figure}{Average Partial Effects under different models.}
    \label{fig:ape_robust}
\end{ThreePartTable}
